Localization-Aware Multi-Scale Representation Learning for Repetitive Action Counting

Repetitive action counting (RAC) aims to estimate the number of class-agnostic action occurrences in a video without exemplars. Most current RAC methods rely on a raw frame-to-frame similarity representation for period prediction. However, this approach can be significantly disrupted by common noise such as action interruptions and inconsistencies, leading to sub-optimal counting performance in realistic scenarios. In this paper, we introduce a foreground localization optimization objective into similarity representation learning to obtain more robust and efficient video features. We propose a Localization-Aware Multi-Scale Representation Learning (LMRL) framework. Specifically, we apply a Multi-Scale Period-Aware Representation (MPR) with a scale-specific design to accommodate various action frequencies and learn more flexible temporal correlations. Furthermore, we introduce the Repetition Foreground Localization (RFL) method, which enhances the representation by coarsely identifying periodic actions and incorporating global semantic information. These two modules can be jointly optimized, resulting in a more discerning periodic action representation. Our approach significantly reduces the impact of noise, thereby improving counting accuracy. Additionally, the framework is designed to be scalable and adaptable to different types of video content. Experimental results on the RepCountA and UCFRep datasets demonstrate that our proposed method effectively handles repetitive action counting.

==> fig/RFL_pipe.tex <==
https://www.canva.cn/design/DAGH5AepVXk/xKmlbiWg2ZIecQo1pPGI5g/edit?utm_content=DAGH5AepVXk&utm_campaign=designshare&utm_medium=link2&utm_source=sharebutton\begin{figure}[]
    \centering
    \includegraphics[width=0.8\linewidth]{img/loc_eccv.png}
    \caption{\textbf{Detailed RFL branch.} Our proposed RFL branch specializes in localizing foreground period of repetitive action video, thereby denoising background information and enhancing representation efficiency.}
    \label{fig:RFL_pipe}
    \vspace{-10pt}
\end{figure}

==> fig/main_pipe.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=0.8\linewidth]{img/main_pipe_eccv.png}
    \caption{\textbf{Framework of our RAC pipline. }Utilizing the extracted video feature as input, our proposed LMRL method, equipped with MPR and RFL branches, enhances the video representation to achieve a more precise prediction. Subsequently, the Counter module maps the strengthened embedding to the density map, incorporating a transformer and two fully connected layers. The primary dimension information is annotated atop the data. For fair comparisons with other methods, the number of sampled frames in our framework is set to 64 by default.}
    \label{fig:main_pipe}
    \vspace{-20pt}
\end{figure}

==> fig/multi_pipe.tex <==
\begin{figure*}[b]
    \centering
    \includegraphics[width=1\linewidth]{img/detai_eccv.png}
    \caption{\textbf{Detailed MPR branch.} Our devised MPR branch captures multi-scale information from the video, effectively addressing action inconsistency. Furthermore, the proposed DSM module, equipped with learnable parameters, computes a similarity matrix, enhancing flexibility in the model's representation.}
    \label{fig:multi_pipe}
    \vspace{-5pt}
\end{figure*}

==> fig/pipeline.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{img/pipeline_eccv4.png}
    \caption{\textbf{An overview of our framework}. First, we use a sliding window to extract video clips and feed them into the backbone. Then, we send the feature $X$ into the dual-branches network. For each scale in the MPR, we calculate the distribution-specific similarity. Then, we apply Max-Pooling to distill information for self-attention. For the RFL, we generate the intermediate result by TCN blocks and take the feature map from the last TCN for further prediction. After several linear projections to adjust dimensions and concatenations, we integrate all the outputs to get a reinforced representation $X^{'}$ for the decoder to predict the density map. Notably, the MPR and RFL branches are supervised by triplet margin loss and localization loss, respectively.}
    \label{fig:pipeline}
    \vspace{-15pt}
\end{figure*}

==> fig/predictedcount.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{img/four_grid.png}
    \caption{\textbf{Predicted Count on the RepCountA benchmark.} (a), (b) and (c) show the distribution of ground truth count, ours model results and TransRAC results respectively, which shows the efficiency of our in handling various action duration. (d) compares the accuracy of our method with TransRAC. }
    \label{fig:statics}
\end{figure}

==> fig/simx.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.8\linewidth]{img/sim4.png}
    \captionsetup{font=small}
    \caption{Various distribution-specific similarity matrices obtained from single video(yellow indicates high similarity,blue means low similarity). }
    \label{fig:simx}
    \vspace{-10pt}
\end{wrapfigure}

==> fig/stu2_39.tex <==
% \begin{figure*}[t]
%     \centering
%     \vspace{-10pt}
%     \includegraphics[height=3cm, width=1\linewidth]{img/12.png}
%     \caption{\textbf{Visualization of MPR on stu2\_39 video.} The top bar labeled ``\textit{GT}" in the graph represents the ground truth density map. the others the outputs from different scales of our MPR. The deeper shade of blue in these bars indicates an elevated numerical magnitude.}
%     \label{fig:visualsim}
%     \vspace{-10pt}
% \end{figure*}
\begin{figure}[]
    \vspace{-10pt}
    \begin{subfigure}
        \centering
        \includegraphics[height=4.2cm,width=1\linewidth]{img/mscal.png}
          % \caption{\textbf{Visualization of MPR.} The ``\textit{GT}" in the graph represents the ground truth density map. The others are the outputs from different scales of our MPR. The deeper shade of blue in these bars indicates an elevated numerical magnitude.}
    \end{subfigure}
    \begin{subfigure}
        \centering
        \includegraphics[height=4.2cm,width=0.85\linewidth]{img/sim4.png}
        % \caption{\textbf{Various similarity matrices obtained from single video.} Distinct weight have been learned to capture similarity information in real-world scenarios. }
    \end{subfigure}
    \caption{\textbf{Visualization of the proposed MPR.} The left side illustrates the output score of the entire MPR module. The ``\textit{GT}'' in the graph represents the ground truth density map. The others represent the outputs from different scales of MPR, showcasing a hierarchy repetition pattern. Meanwhile, the right side displays a collection of diverse similarity matrices acquired from different scales, in which distinct weights have been learned to capture similarity information in real-world video.}
    \label{fig:simx}
    \vspace{-10pt}
\end{figure}



==> fig/supsim1.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-10pt}
    \includegraphics[height=0.7\textwidth, width=0.8\linewidth]{img/12.png}
    \caption{\textbf{Visualization of our proposed MPR.} The uppermost "\textit{GT}"  bar in the graph represents the ground truth density map, while the bars beneath the "\textit{GT}" show the outputs from various scales of our MPR. The deeper shade of blue in these bars indicates an elevated numerical magnitude.}
    \label{fig:visual}
    \vspace{-10pt}
\end{figure*}

==> fig/supsim2.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.8\linewidth]{img/simmapsup.png}
    \caption{\textbf{Visualization of distribution-specific similarity matrix.} In each case, the heatmap shows the similarity score between feature pair at each frame. The red boxes exhibit the distinct weights assigned in each scale from the same video.}
    \label{fig:sim}
    \vspace{-10pt}
\end{figure*}

==> fig/teaser.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{img/teaser_12.png}
    \caption{\textbf{Two challenging cases existing in Repetitive Action Counting (face masked)}. (a) A man squats slower as physical strength declines. The action duration often changes, leading to failure prediction in previous methods due to their single-scale representation. In contrast, we propose a new Localization-Aware-Multi-Scale Representation Learning approach to handle frequency variation. (b) A woman rests between exercise sets. Our proposed methods refine the representation by localizing the foreground interests, shown as continuous repetitive exercising action blocks.}
    \label{fig:teaser}
    \vspace{-15pt}
\end{figure*}


==> sec/0_abstract.tex <==
\begin{abstract}
% 先介绍任务
%Repetitive action counting (RAC) aims to estimate the number of class-agnostic action occurrences in a video with no exemplars, such as physical exercises. 
%再介绍任务的核心问题
%An efficient and accurate method to model and catch its repetitive pattern is essential. 
%以前工作对于核心问题的缺失
%However, previous methods ignored the common noise like interruption and action inconsistencies, etc., resulting in low accuracy in realistic scenarios. 
%我们如何解决
%To complement this margin, we propose a Repetitive-Aware Similarity Representation approach for RAC, which enhances the pre-trained video representation. 
% idea 层面
%Specifically, we regard repetitive action as sequences of frames that share a similar pattern, which could be learned by leveraging context-similarity information. Moreover, we devise a multi-scale repetitive aware framework (MRA) to tackle action inconsistencies. 
%实验结果
%Experimental results in RepCountA and UCFRep datasets demonstrate the effectiveness of the proposed method.
% dong xin comment 
% Experimental results in RepCount and UCFRep datasets demonstrate the effectiveness of the proposed method. 
% dongxin comment 
% Repetitive action counting (RAC) aims to estimate the number of class-agnostic action occurrences in a video with no exemplars, such as physical exercises. Existing methods mainly employ the temporal self-similarity representation for period prediction. However, this constrained representation can be significantly disturbed by the common noise like action interruption and action inconsistencies, which leads to sub-optimal counting performance in realistic scenarios. In this paper, we propose a Repetitive-Aware Similarity Representation (RASR) approach for obtaining the robust period action representation. Specifically, we design a bilateral branch for coarse-to-fine period action localization and multi-scale representation. In the coarse-grained localization branch, period action can be coarsely identified at the instance-level by leveraging global semantic information. In the fine-grained representation branch, we utilize a scale-specific attention mechanism to discriminate the period action embedding and background noise embedding. These two modules can be jointly optimized and result in a discriminated period action representation. Experimental results in RepCount and UCFRep datasets demonstrate that our proposed method can effectively deal with repetitive action counting in the wild.
% dongxin comment 
%Repetitive action counting (RAC) aims to estimate the number of class-agnostic action occurrences in a video with no exemplars, such as physical exercises. Existing methods mainly employ the temporal self-similarity representation for period prediction. However, the constrained representation can be significantly disturbed by common noise like action interruption and action inconsistencies, which leads to sub-optimal counting performance in realistic scenarios. This paper proposes a Dual-Branch Multi-Scale Representation Learning (DMR) approach for zooming into the stable periodic action representation. Specifically, we develop a bilateral branch for coarse-to-fine periodic action localization and multi-scale representation. In the coarse-grained localization branch, periodic action can be coarsely identified at the instance level by leveraging global semantic information. In the fine-grained representation branch, we propose a scale-specific attention mechanism to differentiate between periodic action embeddings and background noise embeddings. These two modules can be jointly optimized, resulting in a more discerning periodic action representation. Experimental results in the RepCount and UCFRep datasets demonstrate that our proposed method can effectively handle repetitive action counting in the wild.

%Sujia Comment
% 1 介绍任务
% Repetitive action counting (RAC) aims to estimate the number of class-agnostic action occurrences in a video with no exemplars, such as physical exercises. Most current RAC methods are based on a raw frame-to-frame similarity representation to present a video, significantly disturbed by interruption and action inconsistencies. However, a distilled representation can potentially strengthen RAC models and make them more noise-sensitive and accurate with more complex scenarios. To improve action representation for RAC, we propose a new representation approach. Specifically, we first apply Multi-Scale Period-Aware Representation (MPR) to guard various action frequencies. Secondly, by using a new Repetition Foreground Localization (RFL) method, periodic action can be coarsely identified at the instance level by leveraging global semantic information. Moreover, our proposed scale-specific attention mechanism is applied to learn a more flexible temporal correlation. These two modules can be jointly optimized, resulting in a more discerning periodic action representation. Experimental results in the RepCount and UCFRep datasets demonstrate that our proposed method can effectively handle repetitive action counting.

%Xiangwei Comment
% 1 介绍任务
Repetitive action counting (RAC) aims to estimate the number of class-agnostic action occurrences in a video with no exemplars. Most current RAC methods are based on a raw frame-to-frame similarity representation for period prediction. However, the constrained representation can be significantly disturbed by common noise like action interruptions and action inconsistencies, which leads to sub-optimal counting performance in realistic scenarios. In this paper, we introduce foreground localization optimization objective into similarity representation learning to obtain more robust and efficient video feature, and propose a Localization-Aware Multi-Scale Representation Learning (LMRL) framework. Specifically, we apply a Multi-Scale Period-Aware Representation (MPR) with scale-specific design to guard various action frequencies and learn a more flexible temporal correlation. Furthermore, we introduce the Repetition Foreground Localization (RFL) method, enhancing the representation by coarsely identifying periodic actions and incorporating global semantic information. These two modules can be jointly optimized, resulting in a more discerning periodic action representation. Experimental results in the RepCountA and UCFRep datasets demonstrate that our proposed method can effectively handle repetitive action counting.
\keywords{Repetitive action counting, Multi-scale representation, Foreground localization, Learnable similarity matrix. }
\end{abstract}
%multi-scale windowed attention  to  scale-specific 

==> sec/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
% dongxin comment 
Repetitive action counting aims to count the number of class-agnostic repetitive actions in a video, which plays a vital role in many applications in human action interpretation \cite{ribnick20103d,huang2016camera}. While a lot of efforts have been devoted to repetitive action counting, the performance of existing temporal self-similarity-based representation methods still needs improvement under diverse action scenes. Figure \ref{fig:teaser} shows two real-life examples of action inconsistency and interruptions, in which the current representation methods neglect. The first subfigure shows a man squatting slower as his strength declines, and the action duration varies from 1.1s to 2.9s; the second subfigure shows a woman doing leg raises and taking a short break in the middle of the exercise sets. Inconsistency and interruption are natural characteristics of actions, usually neglected by previous methods, catastrophically damaging the action intermediate periodic representation and further degrading the performance of period prediction.

%先对现有的方法做一个简单的分类 和related work相对应

In the context of variant repetitive action counting methods, the early methods \cite{levy,pogalin} focus on counting actions from limited cases, such as a synthetic noise square making periodic rotation. These methods count only period uniform actions in short videos and struggles in high variability scenarios. Recently, many challenging datasets and methods have been proposed to make RAC come to fruition \cite{zhang2020context, repnet, hu2022transrac}. A robust periodic representation for repetition action is required to introduce periodic prior. A fixed temporal self-similarity matrix is widely applied in the following works due to its simplicity and generalization ability in unseen repetitions. However, the central issue of this method is that common noise, like action duration inconsistencies, can quickly destroy the temporal self-similarity representation, leading to sub-optimal period prediction. Therefore recent work by Hu et al. \cite{hu2022transrac} tried to solve this problem by applying a multi-scale strategy to the temporal encoder or simply by improving temporal resolution for fine-grained temporal modeling. Nevertheless, these methods still suffer the distraction from action interruption, such as a resting break between two exercise sets shown in Figure \ref{fig:teaser}. Thus, a generic solution is urgently required for both action interruption recognition and various duration perceptions, which outputs robust intermediate periodic representation. 
%In the context of variant repetitive action counting methods, Levy et al. \cite{levy} and Pogalin et al. \cite{pogalin} performed early struggles that held the periodic assumption. Moreover, Dwibedi et al. \cite{repnet} first utilized temporal self-similarity as an intermediate representation for period prediction. This paradigm is widely applied in the following works due to its simplicity and generalization ability in unseen repetitions. However, the major issue of this method is that common noise like action duration inconsistencies can destroy the temporal self-similarity representation easily, leading to sub-optimal period prediction. Recently, Hu et al. \cite{hu2022transrac} and Li et al. \cite{fullresolution} tried to solve this problem by proposing multi-scale temporal encoder or full resolution temporal module for fine-grained temporal modeling. Nevertheless, these methods still suffer the disturbation from action interruption such as break in jumping jack. Thus, a generic solution is urgently required for both action interruption recognition and various duration perception, which outputs robust intermediate periodic representation.
%Pre
% To address the two challenges above, we propose a new Multi-Scale Representation approach for obtaining robust periodic action representation. Firstly, we perform a scale-specific attention mechanism on the temporal self-similarity representation, which can discriminate the periodic action embedding and background noise embedding. Secondly, we take into consideration the coarse-grained dense action localization, by which periodic action can be coarsely identified at the instance level by leveraging global semantic information and action interval annotations. Furthermore, These modules are optimized jointly and yield a fine-grained periodic action representation. To show the effectiveness of the proposed method, we conducted abundant experiments in the RepCount and UCFRep datasets. The experimental results show that our method achieves better periodic prediction than existing methods. 
% Xiangwei 

To address the two challenges mentioned above, we propose a new Localization-Aware Multi-Scale Representation Learning approach for obtaining robust periodic action representation. Firstly, we perform a scale-specific attention mechanism on the temporal self-similarity representation, which can discriminate the periodic action embeddings and background noise embeddings. Secondly, we take into consideration the coarse-grained dense action localization, by which periodic action can be coarsely identified at the instance level by leveraging global semantic information and action interval annotations. Furthermore, these modules are optimized jointly and yield a fine-grained periodic action representation. To show the effectiveness of the proposed method, we conducted abundant experiments in the RepCountA and UCFRep datasets. The experimental results show that our method achieves better periodic prediction than existing methods. 
% The main contributions of our work can be concluded to:
% \begin{enumerate}
% \item Our method features a bilateral branch framework to robust and efficient containing the coarse-to-fine periodic action localization and multi-scale representation. The coarse-grained branch identifies period action at the instance level using global semantic information, while the fine-grained branch employs a scale-specific attention mechanism to distinguish periodic action from background noise. This design can effectively handle the action interruption and inconsistency problems when retrieving repetitive actions in realistic videos.
% \item Extensive experimental results in serveral public datasets demonstrate that our method can effectively deal with repetitive action counting in the wild. 
% \end{enumerate}
%CVPR
% The main contributions of our work can be concluded as follows:
% \begin{enumerate}
% \item We propose a new framework to obtain a robust and efficient representation of repetitive action containing the repetition foreground localization and multi-scale period-aware representation.
% \item Our Multi-Scale Period-Aware Representation presents a novel similarity paradigm for RAC, which extracts information from multiple distinct channels to represent repetitive actions better for realistic scenes with unfixed action length and distribution.
% \item Extensive experimental results in several public datasets demonstrate that our method can effectively deal with repetitive action counting in the wild. 

The main contributions of our work can be concluded as follows:
\begin{enumerate}
\vspace{-0.1em}
\item We propose a robust and efficient representation learning framework to explore repetition in complex scenarios by introducing localization methods. 
\item Our Multi-Scale Period-Aware Representation presents a novel temporal correlation paradigm for RAC, which extracts information from multiple distinct channels to represent repetitive actions better for realistic scenes with unfixed action length and distribution.
\item Extensive experimental results in several public datasets demonstrate that our method can effectively deal with repetitive action counting in the wild.
\vspace{-0.7em}
\end{enumerate}

\input{fig/pipeline}
% %Introduction to this task
% % Task intro
% Repetition Action Counting (RAC) aims to count the number of each class-agnostic repetitive action. 
% % Task Importance
% RAC is critical for understanding human and other physical activities in the wild, assessing exercise performance, and guiding rehabilitation. Humans can easily count actions from most visual action categories for a long time, knowing to pause counting during the break (teaser) and get more focused as the speed goes up. In contrast, the current state-of-the-art method (ref) for counting can only handle constant motion without interruption. It treats counting as a supervised regression task, utilizing thousands of labeled videos to learn a transformer that maps the video representation to its corresponding density map, from which the estimated count is obtained by summing all the density values. As it uses a similarity matrix to model the video representation, each element of which is the similarity value of the features of the corresponding two frames, it first uniform down-samples the video to 64 frames. 
% % Task challenge
% This ignores the noise naturally brought by realistic videos, such as action inconsistency and breaks.
%  %Furthermore, there are a lot of 
%  %potential applications of RepCount. For example, a gym aerobics instructor can interact with the users, and correct and count movement for each group of motions. Robust and precise RepCount algorithms are essential for providing accurate feedback to users, enabling objective assessments, and facilitating personalized fitness programs. In addition, there are other range from organic cycles, such as heartbeats and breathing, through programming and manufacturing, to planetary cycles like the day-night cycle and seasons. Thus the need for recognizing repetitions in videos is pervasive, and a system that is able to identify and count repetitions in video will benefit any perceptual system that aims to observe and understand our world for an extended period of time.
% % Introduce our method
% To this end, we proposed a more robust method for period action representation. Our model features a bilateral branch for coarse-to-fine period action localization and a multi-scale representation. The coarse-grained branch identifies period action at the instance level using global semantic information, while the fine-grained branch employs a multi-scale windowed attention mechanism to distinguish period action from background noise. Together, these modules optimize and yield a discriminated period action representation.
% % conclude the contributions of our work
% The main contributions of our work can be concluded to:
% \begin{enumerate}
%     \item We first adopt a Multi-scale strategy to understand repetition actions based on pre-trained frame-wise feature extraction. It enables the model to explore extensive temporal context, handling the action inconsistency and break situations, which is vital for retrieving repetitive actions in realistic videos.
%     \item Extensive experimental results demonstrate that our method achieves better or comparable performance on three public datasets.
% \end{enumerate}
%-------------------------------------------------------------------------
%\begin{figure*}
  %\centering
  %\begin{subfigure}{0.68\linewidth}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    %\caption{An example of a subfigure.}
    %\label{fig:short-a}
 % \end{subfigure}
  %\hfill
  %\begin{subfigure}{0.28\linewidth}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    %\caption{Another example of a subfigure.}
    %\label{fig:short-b}
  %\end{subfigure}
 % \caption{Example of a short caption, which should be centered.}
  %\label{fig:short}
%\end{figure*}


==> table/dataset.tex <==
\begin{table}[]
\centering
\small
\renewcommand\tabcolsep{2mm}
\caption{\textbf{Dataset statistic of RepCountA and UCFRep}}
\begin{tabular}{l|l|l}
\hline
                    & RepCountA     & UCFRep      \\ \hline
Num.of Videos       & 1041          & 526         \\
Num.of Categories   & 16            & 23          \\
Duration Avg.± Std  & 30.67 ± 17.54 & 8.15 ± 4.29 \\
Duration Min. ± Max & 4.0/88.0      & 2.08/33.84  \\
Count Avg.± Std.    & 14.99 ± 14.70 & 6.66        \\
Count Min. /Max     & 1/141         & 3/54        \\ \hline
\end{tabular}
\label{table:dataset}
\end{table}

==> table/mul.tex <==
\begin{wraptable}{r}{0.48\textwidth}
\vspace{-15pt}
\caption{\textbf{Comparison between ensembling representations and our singular LMRL.}}
\centering


% \begin{tabular}{c|c|c}
% \toprule
%               & \multicolumn{1}{c|}{$ \mathrm{MAE} \downarrow$} & $\mathrm{OBO}\uparrow$             \\ \hline
% Ours & \textbf{0.4200}          & 0.3816          \\
% Ours(Multi)   & 0.4233                   & \textbf{0.4079} \\ \hline
% \end{tabular}
% \end{table}
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{c|cc}
\hline
\multicolumn{1}{l|}{} & \multicolumn{2}{c}{\textbf{RepCountA}}                 \\ \hline
Method                & \multicolumn{1}{c|}{$ \mathrm{MAE} \downarrow$}             & $\mathrm{OBO}\uparrow$               \\ \hline
Ours(4-Scale)        & \multicolumn{1}{c|}{\textbf{0.4200}} & 0.3816          \\
Ours(Multi)           & \multicolumn{1}{c|}{0.4233}          & \textbf{0.4079} \\ \hline
\end{tabular}%
}
\vspace{-15pt}
\label{table:mul}
\end{wraptable}

==> table/spe.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]

% \begin{tabular}{@{}c|c|c@{}}
% \toprule
%         & MAE             & OBO             \\ \midrule
% Without & 0.5172          & 0.3289          \\
% Avg     & 0.4429          & 0.3224          \\
% Max     & \textbf{0.4200} & \textbf{0.3815} \\ \bottomrule
% \end{tabular}
% \end{table}
\begin{wraptable}{r}{0.56\textwidth}
\vspace{-20pt}
\caption{\textbf{Experiment results of different pooling strategy.}}
\centering
\renewcommand\tabcolsep{3.5mm}
\renewcommand\arraystretch{1.1}
\begin{tabular}{l|ll}
\hline
        & \multicolumn{2}{c}{\textbf{RepCountA}}                    \\ \hline
Method  & \multicolumn{1}{l|}{$ \mathrm{MAE} \downarrow$}       & $\mathrm{OBO}\uparrow$            \\ \hline
Without & \multicolumn{1}{l|}{0.5172} &  0.3289                \\
Avg     & \multicolumn{1}{l|}{0.4429}          & 0.3224                \\
Max     & \multicolumn{1}{l|}{\textbf{0.4200}}    & \textbf{0.3816} \\ \hline
\end{tabular}
\label{table:spe}
\vspace{-10pt}
\end{wraptable}
% \begin{tabular}{c|c|c}
% \toprule
%         & $ \mathrm{MAE} \downarrow$     & $\mathrm{OBO}\uparrow$             \\ \hline
% Without & 0.5172          & 0.3289          \\
% Avg     & 0.4429          & 0.3224          \\
% Max     & \textbf{0.4200} & \textbf{0.3815} \\ \hline
% \end{tabular}
% \end{table}\textbf{}
